Sparse Orthogonal Matching Pursuit-based Parameter Estimation for Integrated Sensing and Communications

Accurate parameter estimation such as angle of arrival (AOA) is essential to enhance the performance of integrated sensing and communication (ISAC) in mmWave multiple-input multiple-output (MIMO) systems. This work presents a sensing-aided communication channel estimation mechanism, where the sensing channel shares the same AOA with the uplink communication channel. First, we propose a novel orthogonal matching pursuit (OMP)-based method for coarsely estimating the AOA in a sensing channel, offering improved accuracy compared to conventional methods that rely on rotational invariance techniques. Next, we refine the coarse estimates obtained in the first step by modifying the Space-Alternating Generalized Expectation Maximization algorithm for fine parameter estimation. Through simulations and mathematical analysis, we demonstrate that scenarios with shared AOA achieve a better Cramer-Rao lower bound (CRLB) than those without sharing. This finding highlights the potential of leveraging joint sensing and communication channels to enhance parameter estimation accuracy, particularly in channel or location estimation applications.

==> isac.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,488); %set diagram left start at 0, and has height of 488

%Shape: Axis 2D [id:dp40958542509806595] 
\draw [line width=1.5]  (139.85,163.5) -- (254.39,163.5)(151.3,92.04) -- (151.3,171.44) (247.39,158.5) -- (254.39,163.5) -- (247.39,168.5) (146.3,99.04) -- (151.3,92.04) -- (156.3,99.04)  ;
%Flowchart: Process [id:dp6497156736020778] 
\draw  [line width=1.5]  (144.55,132.5) -- (158.05,132.5) -- (158.05,194.5) -- (144.55,194.5) -- cycle ;
%Straight Lines [id:da11708659763715512] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (151.3,158) -- (239.33,69.44) ;
\draw [shift={(242.15,66.6)}, rotate = 134.83] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (9.29,-4.46) -- (0,0) -- (9.29,4.46) -- cycle    ;
%Straight Lines [id:da37162666420227675] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=1.5]    (262.69,70.32) -- (445.67,103.65) ;
\draw [shift={(258.75,69.6)}, rotate = 10.32] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (9.29,-4.46) -- (0,0) -- (9.29,4.46) -- cycle    ;
%Straight Lines [id:da6875252293384623] 
\draw [color={rgb, 255:red, 43; green, 128; blue, 229 }  ,draw opacity=1 ][line width=1.5]    (156.8,158.5) -- (433.44,104.42) ;
\draw [shift={(437.37,103.65)}, rotate = 168.94] [fill={rgb, 255:red, 43; green, 128; blue, 229 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (9.29,-4.46) -- (0,0) -- (9.29,4.46) -- cycle    ;
%Shape: Circle [id:dp6408630476555244] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (242.15,66.6) .. controls (242.15,71.18) and (245.87,74.9) .. (250.45,74.9) .. controls (255.03,74.9) and (258.75,71.18) .. (258.75,66.6) .. controls (258.75,62.02) and (255.03,58.3) .. (250.45,58.3) .. controls (245.87,58.3) and (242.15,62.02) .. (242.15,66.6) -- cycle ;
%Straight Lines [id:da629128120688324] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (244.3,72.5) -- (158.62,158.66) ;
\draw [shift={(155.8,161.5)}, rotate = 314.84] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (9.29,-4.46) -- (0,0) -- (9.29,4.46) -- cycle    ;
%Straight Lines [id:da9573162528289595] 
\draw [color={rgb, 255:red, 43; green, 128; blue, 229 }  ,draw opacity=1 ][line width=1.5]    (163.73,161.74) -- (439.37,108.65) ;
\draw [shift={(159.8,162.5)}, rotate = 349.1] [fill={rgb, 255:red, 43; green, 128; blue, 229 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (9.29,-4.46) -- (0,0) -- (9.29,4.46) -- cycle    ;
%Straight Lines [id:da9065136994093609] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (156.8,163.5) -- (331.76,247.91) ;
\draw [shift={(335.37,249.65)}, rotate = 205.76] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (9.29,-4.46) -- (0,0) -- (9.29,4.46) -- cycle    ;
%Shape: Circle [id:dp2001981954589629] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (145.8,163.5) .. controls (145.8,166.54) and (148.26,169) .. (151.3,169) .. controls (154.34,169) and (156.8,166.54) .. (156.8,163.5) .. controls (156.8,160.46) and (154.34,158) .. (151.3,158) .. controls (148.26,158) and (145.8,160.46) .. (145.8,163.5) -- cycle ;
%Straight Lines [id:da08485092153206053] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (333,254) -- (159.05,169.74) ;
\draw [shift={(155.45,168)}, rotate = 25.84] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (9.29,-4.46) -- (0,0) -- (9.29,4.46) -- cycle    ;
%Shape: Circle [id:dp1695315353403496] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (332,254) .. controls (332,258.4) and (335.57,261.98) .. (339.98,261.98) .. controls (344.38,261.98) and (347.95,258.4) .. (347.95,254) .. controls (347.95,249.6) and (344.38,246.02) .. (339.98,246.02) .. controls (335.57,246.02) and (332,249.6) .. (332,254) -- cycle ;
%Straight Lines [id:da28416892949392913] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (445.67,103.65) -- (347.81,245.36) ;
\draw [shift={(345.53,248.65)}, rotate = 304.63] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (9.29,-4.46) -- (0,0) -- (9.29,4.46) -- cycle    ;
%Shape: Circle [id:dp8418806804441651] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (437.37,103.65) .. controls (437.37,108.23) and (441.08,111.95) .. (445.67,111.95) .. controls (450.25,111.95) and (453.97,108.23) .. (453.97,103.65) .. controls (453.97,99.07) and (450.25,95.35) .. (445.67,95.35) .. controls (441.08,95.35) and (437.37,99.07) .. (437.37,103.65) -- cycle ;
%Curve Lines [id:da754637096071834] 
\draw  [dash pattern={on 1.5pt off 0.75pt on 0.75pt off 0.75pt}]  (238.45,163.9) .. controls (241.15,157.6) and (242.23,153.73) .. (237.32,147.19) ;
\draw [shift={(235.45,144.9)}, rotate = 48.81] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Curve Lines [id:da22386940015704393] 
\draw  [dash pattern={on 1.5pt off 0.75pt on 0.75pt off 0.75pt}]  (185.45,163.2) .. controls (190.05,155.84) and (188.73,145.09) .. (181.48,136.96) ;
\draw [shift={(179.45,134.9)}, rotate = 42.68] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Curve Lines [id:da6649703226080542] 
\draw  [dash pattern={on 1.5pt off 0.75pt on 0.75pt off 0.75pt}]  (213.45,163.2) .. controls (218.97,172.4) and (218.57,180.75) .. (210.68,188.26) ;
\draw [shift={(208.45,190.2)}, rotate = 321.34] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Shape: Axis 2D [id:dp45402928204503423] 
\draw [line width=1.5]  (460.02,103.65) -- (316.48,103.65)(445.67,22.66) -- (445.67,112.65) (323.48,98.65) -- (316.48,103.65) -- (323.48,108.65) (450.67,29.66) -- (445.67,22.66) -- (440.67,29.66)  ;
%Curve Lines [id:da2441820117519089] 
\draw  [dash pattern={on 1.5pt off 0.75pt on 0.75pt off 0.75pt}]  (396.58,104.6) .. controls (396.58,122.46) and (403.65,131.48) .. (416.96,138.32) ;
\draw [shift={(419.58,139.6)}, rotate = 205.02] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Curve Lines [id:da31483572266942117] 
\draw  [dash pattern={on 1.5pt off 0.75pt on 0.75pt off 0.75pt}]  (361.58,103.6) .. controls (358.16,112.15) and (359.86,117.04) .. (363.55,121.41) ;
\draw [shift={(365.58,123.6)}, rotate = 225] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Curve Lines [id:da2525082535010189] 
\draw  [dash pattern={on 1.5pt off 0.75pt on 0.75pt off 0.75pt}]  (343.58,103.6) .. controls (341.76,93.59) and (341.71,96.58) .. (344.63,88.38) ;
\draw [shift={(345.58,85.6)}, rotate = 108.29] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;

% Text Node
\draw (239,30) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{T}_{1}$};
% Text Node
\draw (101,141) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{26.52pt}\setlength\topsep{0pt}
ISAC
\begin{center}
BS
\end{center}

\end{minipage}};
% Text Node
\draw (414,74) node [anchor=north west][inner sep=0.75pt]   [align=left] {UE};
% Text Node
\draw (340,65) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$d_{k,1}$};
% Text Node
\draw (178,88) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$d_{k,2}$};
% Text Node
\draw (296.08,133.07) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$d_{0}$};
% Text Node
\draw (322.12,101.79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-0.59]  {$\theta _{\text{Tx} ,0}$};
% Text Node
\draw (307.12,78.79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-0.59]  {$\theta _{\text{Tx} ,1}$};
% Text Node
\draw (376.12,121.79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-0.59]  {$\theta _{\text{Tx} ,2}$};
% Text Node
\draw (248.48,143.25) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-0.59]  {$\theta _{\text{Rx} ,0}$};
% Text Node
\draw (142,67) node [anchor=north west][inner sep=0.75pt]   [align=left] {y};
% Text Node
\draw (258,161) node [anchor=north west][inner sep=0.75pt]   [align=left] {x};
% Text Node
\draw (187.12,126.79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-0.59]  {$\theta _{\text{Rx} ,1}$};
% Text Node
\draw (219.12,169.79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-0.59]  {$\theta _{\text{Rx} ,2}$};
% Text Node
\draw (384,184) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$d_{k,1}$};
% Text Node
\draw (214,207) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$d_{k,2}$};
% Text Node
\draw (360,235) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{T}_{2}$};
% Text Node
\draw (451,72) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{T}_{0}$};


\end{tikzpicture}

